Large Language Model-based Human-Agent Collaboration for Complex Task Solving

In recent developments within the research community, the integration of Large Language Models (LLMs) in creating fully autonomous agents has garnered significant interest. Despite this, LLM-based agents frequently demonstrate notable shortcomings in adjusting to dynamic environments and fully grasping human needs. In this work, we introduce the problem of LLM-based human-agent collaboration for complex task-solving, exploring their synergistic potential. In addition, we propose a Reinforcement Learning-based Human-Agent Collaboration method, ReHAC. This approach includes a policy model designed to determine the most opportune stages for human intervention within the task-solving process. We construct a human-agent collaboration dataset to train this policy model in an offline reinforcement learning environment. Our validation tests confirm the model's effectiveness. The results demonstrate that the synergistic efforts of humans and LLM-based agents significantly improve performance in complex tasks, primarily through well-planned, limited human intervention. Datasets and code are available at: https://github.com/XueyangFeng/ReHAC.

==> sections/data_collection.tex <==


\subsection{State formulation}
For question answering datasets, each state \(s_t\) is obtained by agent or human under ReAct (\citet{yao2022react}) framework. Specifically, each state \(a_t\) contains three sequential steps: \textit{Thought}, \textit{Action}, and \textit{Observation}. In the \textit{Thought} step, agent or human needs to reason over the current state and plan the next step action. In the \textit{Action} step, agent or human carries out actions based on the thought in the previous step. Action spaces are constrained to 1) \textbf{search}[entity], which searches the entity wiki page and gains the first 5 sentences from the page. 2) \textbf{lookup}[keyword], which searches the next sentence containing the keyword in the current wiki page. 3) \textbf{finish}[answer], which submits the answer. We use a Wikipedia web API following original ReAct (\citet{yao2022react}) implementation to support all actions. Finally, in the \textit{Observation} step, Wikipedia web API returns results corresponding to the action. If the action \textbf{finish} is conducted, or agent or human fails to act \textbf{finish} within the given step, the trajectory is ended and we will receive final scores. 

For InterCode dataset, we use "Try Again" (\citet{yang2023intercode}) to obtain the state \(s_t\). In "Try Again", each state \(s_t\) comprises two steps: \textit{Action} and \textit{Observation}. Agent or human continually interact with the environment by \textit{Action} and receive the execution output of the \textit{Action} as \textit{Observation}. The interaction continues until the query is completed (the reward from the code environment is 1) or the interaction turns exceeds a predefined threshold. 

\subsection{Data Collection details}
% hotpotqa 采样23条  intercode采样25条
% 这里面需要雪扬写上我们怎么通过马尔可夫采样然后算advantage 函数的

\paragraph{Reward Computing}
For question answering datasets, we use f1 score which evaluates the alignment between the predicted answer and the gold answer as the trajectory reward.
For InterCode datasets, we use the reward from the code environment as the trajectory reward.

==> sections/preliminary.tex <==
\paragraph{LLM-powered Agent}~We formalize the task completion process of agents powered by Large Language Models (LLMs) as a Markov Decision Process (MDP), which is defined by the tuple \((S, A, P, R, \gamma)\). Here, \(S\) represents the set of all possible states, \(A\) denotes the set of all possible actions, \(P\) is the transition probability matrix defining the probability of transitioning from one state to another given an action, \(R\) is the reward function assigning a numerical reward to each state-action pair, and \(\gamma\) is the discount factor that balances the importance of immediate and future rewards.  For each time step \(t\), the action \(a_t\) is determined by the LLM based on the current state \(s_t\), denoted as \(a_t = \text{LLM}(s_t)\). The probability of transitioning to the next state \(s_{t+1}\) given the current state \(s_t\) and action \(a_t\) is defined by the state transition model \(P\), expressed as \(P(s_{t+1} | s_t, a_t)\). The reward \(r_t\) for taking action \(a_t\) in state \(s_t\) is given by the reward function \(R\), expressed as \(r_t = R(s_t, a_t)\).

\paragraph{Constrained Reinforcement Learning}~In our study, we aim to develop a decision model that balances rewards and costs in human-machine collaboration. This task can be formalized as a Constrained Reinforcement Learning (CRL) problem. CRL is modeled using a Constrained Markov Decision Process (CMDP), an extension of the standard MDP. A CMDP is defined by the tuple \((S, A, P, R, C, \gamma)\), where \(C\) denotes the constraints to be adhered to during decision-making. At each time step \(t\), the agent selects an action \(a_t\) based on the current state \(s_t\), aiming to maximize rewards while satisfying constraints. This process can be formalized as:
\begin{align}
\max_{\theta} \, &\mathbb{E}_{\tau \sim \pi_\theta} [R(\tau)], \\
\text{subject to} \, &\mathbb{E}_{\tau \sim \pi_\theta} [C(\tau)] \leq d.
\end{align}
In the formalized CRL model, \(\theta\) denotes the parameters of the policy \(\pi_\theta\). This policy determines action probabilities in given states. The term \(\mathbb{E}_{\tau \sim \pi_\theta} [R(\tau)]\) is the expected reward, maximized over the trajectory \(\tau\), a sequence of states and actions under the policy. The constraint \(\mathbb{E}_{\tau \sim \pi_\theta} [C(\tau)] \leq d\) ensures the expected cost does not exceed a limit \(d\), balancing reward pursuit with necessary constraints, crucial for sustainable decision-making in human-machine collaboration.







